Should All Cross-Lingual Embeddings Speak English?

Most of recent work in cross-lingual word embeddings is severely Anglocentric. The vast majority of lexicon induction evaluation dictionaries are between English and another language, and the English embedding space is selected by default as the hub when learning in a multilingual setting. With this work, however, we challenge these practices. First, we show that the choice of hub language can significantly impact downstream lexicon induction performance. Second, we both expand the current evaluation dictionary collection to include all language pairs using triangulation, and also create new dictionaries for under-represented languages. Evaluating established methods over all these language pairs sheds light into their suitability and presents new challenges for the field. Finally, in our analysis we identify general guidelines for strong cross-lingual embeddings baselines, based on more than just Anglocentric experiments.

==> directionality.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{ccccc}
    \toprule
        Pair & prec@1 & Pair & prec@1 & Diff.\\
    \midrule
        spa--aze & 9.9 & aze--spa & 44.9 & 35.0 \\
        por--aze & 5.3 & aze--por & 39.8 & 34.5 \\
        spa--bel & 10.1 & bel--spa & 39.5 & 29.4 \\
        slk--aze & 3.1 & aze--slk & 31.7 & 28.6 \\
        rus--bel & 12.8 & bel--rus & 41.1 & 28.3 \\
        ces--aze & 6.9 & aze--ces & 34.8 & 27.9 \\
        glg--aze & 5.0 & aze--glg & 32.7 & 27.8\\
        ces--bel & 9.3 & bel--ces & 35.9 & 26.5 \\
        por--bel & 8.6 & bel--por & 34.4 & 25.8 \\
        tur--aze & 8.4 & aze--tur & 32.0 & 23.8 \\
    \bottomrule
    \end{tabular}
    \caption{Evaluating on low--high resource pairs leads to much higher results than high--low pairs.}
    \label{tab:directionality}
\end{table}

==> gh.tex <==
\begin{table}[t]
    %\vspace{-5mm}
    \centering
    \caption{The downstream accuracy generally correlates positively with the GH distance of the source and target language vector spaces to the hub language. \gn{Maybe this could be a figure?}}
    \label{tab:gh}
    \begin{tabular}{@{}c|cccccccccc|c@{}}
    \toprule
        Test Set & \multicolumn{10}{|c}{Hub language} & Corr.\\
        %Set & \az & \be & \cs & \en & \es & \gl & \pt & \ru & \sk & \tr & Coeff.\\
    \midrule
        \gl--\en & \az & \be & \cs & \en & \es & \gl & \pt & \ru & \sk & \tr\\
        P@1 & 40.3 & 41.8 & 41.9 & 39.6 & \textbf{43.2} & 40.8 & 41.5 & 41.9 & 41.6 & 42.1 \\
        $\text{GH}^{hub}_\gl + \text{GH}^{hub}_\en$ & 
        1.22 & 1.85 & 1.65 & 0.90 & 1.37 & 0.90 & 1.15 & 1.71 & 1.61 & 1.63 & 0.73 \\
    \midrule
        \en--\hi & \en & \fr & \hi & \ko & \ru & \sv & \uk & & & & \\
        P@1 & 20.9 & 23.5 & 21.0 & 21.4 & 23.5 & 21.4 & \textbf{23.9} & & & & \\
        $\text{GH}^{hub}_\en + \text{GH}^{hub}_\hi$ & 0.98 & 1.7 & 0.98 & 1.15 & 1.8 & 1.6 & 1.7 & & & & 0.87\\
    \bottomrule
    \end{tabular}
    %\vspace{-4mm}
\end{table}

==> optimal_per_lang.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{cp{5cm}}
    \toprule
        language & optimal alignment languages\\
    \midrule
    spa & eng (21\%)\\
    eng & spa (30\%)\\
    tur & ces (22\%)\\
    por & eng (27\%), spa (22\%)\\
    ces & spa (20\%), por (20\%)\\
    glg & spa (31\%), tur (21\%)\\
    rus & glg (28\%), tur (24\%)\\
    slk & spa (25\%), ces (20\%)\\
    bel & rus (20\%)\\
    aze & por (20\%)\\
    \bottomrule
    \end{tabular}
    \caption{Optimal Alignment languages for each language (regardless of direcionality).}
    \label{tab:best_perlang}
\end{table}

==> stash.tex <==
\iffalse
\paragraph{Does directionality matter?}
%\input{directionality.tex}
\an{Might remove this section. Thoughts?} \gn{Seems reasonable. It seems that this can also be explained just by the fact that translation from English into Azerbaijani is hard, because many Azerbaijani morphological variants might correspond to a single English word.}
We also explore whether there are significant differences between the evaluated quality of aligned spaces, when computed on both directions (src--trg and trg--src).
We find that the evaluation direction indeed has a significant effect; when the languages of the evaluation pair are very distant, in terms of morphological complexity and data availability (which affects the quality of the original embeddings).
A prominent example, from our~10-languages experiment, are evaluation pairs involving \az{} or \be{}.
When evaluating on the \az--XX and \be--XX dictionaries, the word translation P@1 is more than 20 percentage points higher than when evaluating on the opposite direction (XX-\az{} or XX-\be{}). For example, \es--\az{} has a mere P@1 of 9.9, while \az--\es{} achieves a P@1 of 44.9. This observation holds even between very related languages (cf. \ru--\be{}: 12.8, \be--\ru{}: 41.1 and \tr--\az: 8.4, \az--\tr: 32.0), which supports our hypothesis that this difference is also due to the quality of the pre-trained embeddings. It is important to note that such directionality differences are not observed  when evaluating distant pairs with presumably high-quality pre-trained embeddings e.g. \tr--\sk{} or \tr--\es{}; the P@1 for both directions is very close.
\fi

==> surprise.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{cc}
    \toprule
        Best target & Percentage \\
        language &  (over 90 pairs)\\
    \midrule
        src & 4.4\% \\
        trg & 2.2\% \\
        neither & 93.3\% \\
    \bottomrule
    \end{tabular}
    \caption{The optimal target language for aligning $l_{src}$ and $l_{trg}$ is almost always a \textbf{third} language.}
    \label{tab:surprise}
\end{table}
